A Criterion for Post-Selected Quantum Advantage

Assuming the polynomial hierarchy is infinite, we prove a sufficient condition for determining if uniform and polynomial size quantum circuits over a non-universal gate set are not efficiently classically simulable in the weak multiplicative sense. Our criterion exploits the fact that subgroups of $\mathrm{SL}(2;\mathbb{C})$ are essentially either discrete or dense in $\mathrm{SL}(2;\mathbb{C})$. Using our criterion, we give a new proof that both instantaneous quantum polynomial (IQP) circuits and conjugated Clifford circuits (CCCs) afford a quantum advantage. We also prove that both commuting CCCs and CCCs over various fragments of the Clifford group afford a quantum advantage, which settles two questions of Bouland, Fitzsimons, and Koh. Our results imply that circuits over just $(U^\dagger \otimes U^\dagger) \mathrm{CZ} (U \otimes U)$ afford a quantum advantage for almost all $U \in \mathrm{U}(2)$.

==> classification_dependency_diagram.tex <==
\makeatletter

\pgfdeclareshape{bicolor rectangle}
{
    % This bit from \pgflibraryshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{north east}
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{south east}

    \inheritbackgroundpath[from=rectangle]
    \inheritbeforebackgroundpath[from=rectangle]
    \inheritbehindforegroundpath[from=rectangle]
    \inheritforegroundpath[from=rectangle]
    \inheritbeforeforegroundpath[from=rectangle]

   % Now do the background filling.
    \behindbackgroundpath{%
        % \southwest and \northeast defined by rectangle, but
        % (somewhat annoyingly) not \southeast and \northwest
        % so use this workaround.
        \pgfextractx{\pgf@xa}{\southwest}%
        \pgfextracty{\pgf@ya}{\southwest}%
        \pgfextractx{\pgf@xb}{\northeast}%
        \pgfextracty{\pgf@yb}{\northeast}%
				\pgf@xc=.5\pgf@xa%
				\advance\pgf@xc by .5\pgf@xb%
				\pgf@yc=.5\pgf@xa%
				\advance\pgf@yc by .5\pgf@xb%
 
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@left@color}%
        \pgfusepath{fill}%
       
        \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
				\pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
        \pgfpathclose
        
        \color{\pgf@right@color}%
        \pgfusepath{fill}%
    }
}


\pgfdeclareshape{tricolor rectangle}
{
    % This bit from \pgflibraryshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{north east}
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{south east}

    \inheritbackgroundpath[from=rectangle]
    \inheritbeforebackgroundpath[from=rectangle]
    \inheritbehindforegroundpath[from=rectangle]
    \inheritforegroundpath[from=rectangle]
    \inheritbeforeforegroundpath[from=rectangle]

   % Now do the background filling.
    \behindbackgroundpath{%
        % \southwest and \northeast defined by rectangle, but
        % (somewhat annoyingly) not \southeast and \northwest
        % so use this workaround.
        \pgfextractx{\pgf@xa}{\southwest}%
        \pgfextracty{\pgf@ya}{\southwest}%
        \pgfextractx{\pgf@xb}{\northeast}%
        \pgfextracty{\pgf@yb}{\northeast}%
				\pgf@xc=.66\pgf@xa%
				\advance\pgf@xc by .34\pgf@xb%
				\pgf@yc=.34\pgf@xa%
				\advance\pgf@yc by .66\pgf@xb%
 
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@left@color}%
        \pgfusepath{fill}%
       

        \pgfpathmoveto{\pgfpoint{\pgf@yc}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@right@color}%
        \pgfusepath{fill}%
        
        
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}%
        \pgfpathclose
        \color{\pgf@top@color}%
        \pgfusepath{fill}%
    }
}

\def\pgf@top@color{gray!30}
\def\pgf@left@color{gray!30}
\def\pgf@right@color{gray!30}

% Use these with PGF
\def\pgfsetleftcolor#1{\def\pgf@left@color{#1}}%
\def\pgfsetrightcolor#1{\def\pgf@right@color{#1}}%
\def\pgfsettopcolor#1{\def\pgf@top@color{#1}}%

% Use these with TikZ
\tikzoption{left color}{\pgfsetleftcolor{#1}}
\tikzoption{right color}{\pgfsetrightcolor{#1}}
\tikzoption{top color}{\pgfsettopcolor{#1}}
 
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{landscape}\centering
\vspace*{\fill}
\begin{figure}[htpb]
% \begin{sidewaysfigure}
\begin{center}
\begin{tikzpicture}[>=latex]
\tikzstyle{class}=[rectangle, thick, align=center, draw, font=\small, fill=white]
\tikzstyle{xpres}=[class,fill=red!20]
\tikzstyle{ypres}=[class,fill=green!20]
\tikzstyle{zpres}=[class,fill=blue!20] 
%\tikzstyle{nonpres}=[class, fill=black!10]
%\tikzstyle{xypres}=[class, fill=yellow!20]
%\tikzstyle{yzpres}=[class, fill=cyan!20]
%\tikzstyle{xzpres}=[class, fill=purple!20]
%\tikzstyle{xyzpres}=[class, fill=white]
\tikzstyle{nonpres}=[class]
\tikzstyle{xypres}=[class, bicolor rectangle,
        left color=red!20,
        right color=green!20, fill=none]
\tikzstyle{yzpres}=[class, bicolor rectangle,
        left color=green!20,
        right color=blue!20,
        fill=none]
\tikzstyle{xzpres}=[class, bicolor rectangle,
        right color=red!20,
        left color=blue!20,
        fill=none]
\tikzstyle{xyzpres}=[class, tricolor rectangle, 
         top color=green!20,
         left color=red!20,
         right color=blue!20, fill=none]
\matrix[row sep=1.3cm,column sep=.07cm] {
& & & & & \node (criterion) [nonpres]{\thmref{thm:maintwo} (our criterion)}; & & & & &\\
& & & \node (lemmas1) [nonpres]{\lemref{lem:czz_lem_one}}; & & \node (c1) [nonpres]{\lemref{lem:czz_lem_two}}; & & & & &\\
& & \node (lemmas2) [nonpres]{Lemmas~\ref{lem:czz_lem_one}, \ref{lem:czequivalence}, \ref{lem:CZlemma}}; & & & \node (czz) [nonpres]{\thmref{thm:cz+zclassification} ($\CZ + Z$)}; & & \node (lemmas3) [nonpres]{Lemmas~\ref{lem:czz_lem_one}, \ref{lem:czs_lem_one}, \ref{lem:czs_lem_two}}; & & &\\
& & & \node (cz) [nonpres]{\thmref{thm:czclassification} ($\CZ$)}; & & & & \node (czs) [nonpres]{\thmref{thm:cz+sclassification} ($\CZ + S$)}; & & &\\
& & \node (cp) [nonpres]{\thmref{thm:hardness_fragmentfour} ($C(P,P)$)}; & & & & & \node (cprp) [nonpres]{\thmref{thm:hardness_fragmentone} ($C(P,P) + R_P$)}; & & &\\
& & \node (a1) [nonpres]{\lemref{lem:CCC_lem_one}}; & \node (a2) [nonpres]{\lemref{lem:CCC_lem_two}}; & & \node (cpp) [nonpres]{\thmref{thm:hardness_fragmentthree} ($C(P,P) + P$)}; & & & & &\\
& & \node (ccc) [nonpres]{\thmref{thm:CCC_classification} (CCCs)}; & & & & & & & &\\
};

%\coordinate[above left=1cm of CXZ_P.north] (LEFT);
%\coordinate[below right=1cm of CXZ_P_Rz.south] (RIGHT);

% EDGES
\path[draw] 
(criterion) edge[->] (c1)
(c1) edge[->] (czz)
(c1) edge[->] (czs)
(lemmas1) edge[->] (czz)
(lemmas2) edge[->] (cz)
(lemmas3) edge[->] (czs)
(czz) edge[->] (cpp)
(czz) edge[->] (cz)
(czz) edge[->] (czs)
(cz) edge[->] (cp)
(czs) edge[->] (cprp)
(czz) edge[->] (a2)
(a2) edge[->] (ccc)
(a1) edge[->] (ccc);

\end{tikzpicture}

\end{center}
\caption{A dependency diagram for our classification results, where an arrow from A to B means ``A is used in the proof of B''.}
\label{fig:classification_dependency}
% \end{sidewaysfigure}
\end{figure}
\vfill
\end{landscape}

==> hardness_dependency_diagram.tex <==
\makeatletter

\pgfdeclareshape{bicolor rectangle}
{
    % This bit from \pgflibraryshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{north east}
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{south east}

    \inheritbackgroundpath[from=rectangle]
    \inheritbeforebackgroundpath[from=rectangle]
    \inheritbehindforegroundpath[from=rectangle]
    \inheritforegroundpath[from=rectangle]
    \inheritbeforeforegroundpath[from=rectangle]

   % Now do the background filling.
    \behindbackgroundpath{%
        % \southwest and \northeast defined by rectangle, but
        % (somewhat annoyingly) not \southeast and \northwest
        % so use this workaround.
        \pgfextractx{\pgf@xa}{\southwest}%
        \pgfextracty{\pgf@ya}{\southwest}%
        \pgfextractx{\pgf@xb}{\northeast}%
        \pgfextracty{\pgf@yb}{\northeast}%
				\pgf@xc=.5\pgf@xa%
				\advance\pgf@xc by .5\pgf@xb%
				\pgf@yc=.5\pgf@xa%
				\advance\pgf@yc by .5\pgf@xb%
 
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@left@color}%
        \pgfusepath{fill}%
       
        \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
				\pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
        \pgfpathclose
        
        \color{\pgf@right@color}%
        \pgfusepath{fill}%
    }
}


\pgfdeclareshape{tricolor rectangle}
{
    % This bit from \pgflibraryshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{north east}
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{south east}

    \inheritbackgroundpath[from=rectangle]
    \inheritbeforebackgroundpath[from=rectangle]
    \inheritbehindforegroundpath[from=rectangle]
    \inheritforegroundpath[from=rectangle]
    \inheritbeforeforegroundpath[from=rectangle]

   % Now do the background filling.
    \behindbackgroundpath{%
        % \southwest and \northeast defined by rectangle, but
        % (somewhat annoyingly) not \southeast and \northwest
        % so use this workaround.
        \pgfextractx{\pgf@xa}{\southwest}%
        \pgfextracty{\pgf@ya}{\southwest}%
        \pgfextractx{\pgf@xb}{\northeast}%
        \pgfextracty{\pgf@yb}{\northeast}%
				\pgf@xc=.66\pgf@xa%
				\advance\pgf@xc by .34\pgf@xb%
				\pgf@yc=.34\pgf@xa%
				\advance\pgf@yc by .66\pgf@xb%
 
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@left@color}%
        \pgfusepath{fill}%
       

        \pgfpathmoveto{\pgfpoint{\pgf@yc}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@right@color}%
        \pgfusepath{fill}%
        
        
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}%
        \pgfpathclose
        \color{\pgf@top@color}%
        \pgfusepath{fill}%
    }
}

\def\pgf@top@color{gray!30}
\def\pgf@left@color{gray!30}
\def\pgf@right@color{gray!30}

% Use these with PGF
\def\pgfsetleftcolor#1{\def\pgf@left@color{#1}}%
\def\pgfsetrightcolor#1{\def\pgf@right@color{#1}}%
\def\pgfsettopcolor#1{\def\pgf@top@color{#1}}%

% Use these with TikZ
\tikzoption{left color}{\pgfsetleftcolor{#1}}
\tikzoption{right color}{\pgfsetrightcolor{#1}}
\tikzoption{top color}{\pgfsettopcolor{#1}}
 
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{landscape}\centering
\vspace*{\fill}
\begin{figure}[htpb]
% \begin{sidewaysfigure}
\begin{center}
\begin{tikzpicture}[>=latex]
\tikzstyle{class}=[rectangle, thick, align=center, draw, font=\small, fill=white]
\tikzstyle{xpres}=[class,fill=red!20]
\tikzstyle{ypres}=[class,fill=green!20]
\tikzstyle{zpres}=[class,fill=blue!20] 
%\tikzstyle{nonpres}=[class, fill=black!10]
%\tikzstyle{xypres}=[class, fill=yellow!20]
%\tikzstyle{yzpres}=[class, fill=cyan!20]
%\tikzstyle{xzpres}=[class, fill=purple!20]
%\tikzstyle{xyzpres}=[class, fill=white]
\tikzstyle{nonpres}=[class]
\tikzstyle{xypres}=[class, bicolor rectangle,
        left color=red!20,
        right color=green!20, fill=none]
\tikzstyle{yzpres}=[class, bicolor rectangle,
        left color=green!20,
        right color=blue!20,
        fill=none]
\tikzstyle{xzpres}=[class, bicolor rectangle,
        right color=red!20,
        left color=blue!20,
        fill=none]
\tikzstyle{xyzpres}=[class, tricolor rectangle, 
         top color=green!20,
         left color=red!20,
         right color=blue!20, fill=none]
\matrix[row sep=1.3cm,column sep=.07cm] {
& & & \node (criterion) [nonpres]{\thmref{thm:maintwo} (our criterion)}; && & & & & &\\
& \node (b1) [nonpres]{\lemref{lem:czz_lem_one}}; & \node (c1) [nonpres]{\lemref{lem:czz_lem_two}}; & & & \node (ccc) [nonpres]{\thmref{thm:CCC_hardness} (CCCs)}; & \node (iqp) [nonpres]{\thmref{thm:IQP_hardness} (IQP)}; & & & &\\
& & \node (czz) [nonpres]{\thmref{thm:czclassification} ($\CZ + Z$ class.)}; & & & \node (czzhard) [nonpres]{\thmref{thm:czzhardnessresult} ($\CZ + Z$)}; & \node (lemma) [nonpres]{\lemref{lem:CZlemma}}; & & & &\\
& & \node (cpp) [nonpres]{\thmref{thm:hardness_fragmentthree} ($C(P,P) + P$ class.)}; & \node (t4p) [nonpres]{\thmref{thm:t4hardness} ($\T_4 + \Pauli$)};  & & \node (cz) [nonpres]{\thmref{thm:CZhardness} ($\CZ$)}; & & & & &\\
& & \node (fragments) [nonpres]{\thmref{thm:hardness_fragmenttwo} (all Clifford fragments)}; & & & & & & & &\\
};

%\coordinate[above left=1cm of CXZ_P.north] (LEFT);
%\coordinate[below right=1cm of CXZ_P_Rz.south] (RIGHT);

% EDGES
\path[draw] 
(criterion) edge[->] (iqp)
(criterion) edge[->] (ccc)
(criterion) edge[->] (czzhard)
(criterion) edge[->] (t4p)
(criterion) edge[->] (c1)
(b1) edge[->] (czz)
(c1) edge[->] (czz)
(czz) edge[->] (cpp)
(czzhard) edge[->] (cz)
(lemma) edge[->] (cz)
(cpp) edge[->] (fragments)
(t4p) edge[->] (fragments);

\end{tikzpicture}

\end{center}
\caption{A dependency diagram for our hardness results, where an arrow from A to B means ``A is used in the proof of B'' and ``class.'' means the associated theorem is a classification result.}
\label{fig:hardness_dependency}
% \end{sidewaysfigure}
\end{figure}
\vfill
\end{landscape}

==> multi_qubit_lattice.tex <==
\makeatletter

\pgfdeclareshape{bicolor rectangle}
{
    % This bit from \pgflibraryshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{north east}
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{south east}

    \inheritbackgroundpath[from=rectangle]
    \inheritbeforebackgroundpath[from=rectangle]
    \inheritbehindforegroundpath[from=rectangle]
    \inheritforegroundpath[from=rectangle]
    \inheritbeforeforegroundpath[from=rectangle]

   % Now do the background filling.
    \behindbackgroundpath{%
        % \southwest and \northeast defined by rectangle, but
        % (somewhat annoyingly) not \southeast and \northwest
        % so use this workaround.
        \pgfextractx{\pgf@xa}{\southwest}%
        \pgfextracty{\pgf@ya}{\southwest}%
        \pgfextractx{\pgf@xb}{\northeast}%
        \pgfextracty{\pgf@yb}{\northeast}%
				\pgf@xc=.5\pgf@xa%
				\advance\pgf@xc by .5\pgf@xb%
				\pgf@yc=.5\pgf@xa%
				\advance\pgf@yc by .5\pgf@xb%
 
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@left@color}%
        \pgfusepath{fill}%
       
        \pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@yb}}%
				\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
				\pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
        \pgfpathclose
        
        \color{\pgf@right@color}%
        \pgfusepath{fill}%
    }
}


\pgfdeclareshape{tricolor rectangle}
{
    % This bit from \pgflibraryshapes.code.tex
    \inheritsavedanchors[from=rectangle]
    \inheritanchorborder[from=rectangle]
    \inheritanchor[from=rectangle]{north}
    \inheritanchor[from=rectangle]{north west}
    \inheritanchor[from=rectangle]{north east}
    \inheritanchor[from=rectangle]{center}
    \inheritanchor[from=rectangle]{west}
    \inheritanchor[from=rectangle]{east}
    \inheritanchor[from=rectangle]{mid}
    \inheritanchor[from=rectangle]{mid west}
    \inheritanchor[from=rectangle]{mid east}
    \inheritanchor[from=rectangle]{base}
    \inheritanchor[from=rectangle]{base west}
    \inheritanchor[from=rectangle]{base east}
    \inheritanchor[from=rectangle]{south}
    \inheritanchor[from=rectangle]{south west}
    \inheritanchor[from=rectangle]{south east}

    \inheritbackgroundpath[from=rectangle]
    \inheritbeforebackgroundpath[from=rectangle]
    \inheritbehindforegroundpath[from=rectangle]
    \inheritforegroundpath[from=rectangle]
    \inheritbeforeforegroundpath[from=rectangle]

   % Now do the background filling.
    \behindbackgroundpath{%
        % \southwest and \northeast defined by rectangle, but
        % (somewhat annoyingly) not \southeast and \northwest
        % so use this workaround.
        \pgfextractx{\pgf@xa}{\southwest}%
        \pgfextracty{\pgf@ya}{\southwest}%
        \pgfextractx{\pgf@xb}{\northeast}%
        \pgfextracty{\pgf@yb}{\northeast}%
				\pgf@xc=.66\pgf@xa%
				\advance\pgf@xc by .34\pgf@xb%
				\pgf@yc=.34\pgf@xa%
				\advance\pgf@yc by .66\pgf@xb%
 
        \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@left@color}%
        \pgfusepath{fill}%
       

        \pgfpathmoveto{\pgfpoint{\pgf@yc}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathclose
        
        \color{\pgf@right@color}%
        \pgfusepath{fill}%
        
        
        \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}%
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@yb}}%\
        \pgfpathlineto{\pgfpoint{\pgf@yc}{\pgf@ya}}%
        \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}%
        \pgfpathclose
        \color{\pgf@top@color}%
        \pgfusepath{fill}%
    }
}

\def\pgf@top@color{gray!30}
\def\pgf@left@color{gray!30}
\def\pgf@right@color{gray!30}

% Use these with PGF
\def\pgfsetleftcolor#1{\def\pgf@left@color{#1}}%
\def\pgfsetrightcolor#1{\def\pgf@right@color{#1}}%
\def\pgfsettopcolor#1{\def\pgf@top@color{#1}}%

% Use these with TikZ
\tikzoption{left color}{\pgfsetleftcolor{#1}}
\tikzoption{right color}{\pgfsetrightcolor{#1}}
\tikzoption{top color}{\pgfsettopcolor{#1}}
 
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{landscape}\centering
\vspace*{\fill}
\begin{figure}[htpb]
% \begin{sidewaysfigure}
\begin{center}
\begin{tikzpicture}[>=latex]
\tikzstyle{class}=[rectangle, thick, align=center, draw, font=\tiny, fill=white]
\tikzstyle{xpres}=[class,fill=red!20]
\tikzstyle{ypres}=[class,fill=green!20]
\tikzstyle{zpres}=[class,fill=blue!20] 
%\tikzstyle{nonpres}=[class, fill=black!10]
%\tikzstyle{xypres}=[class, fill=yellow!20]
%\tikzstyle{yzpres}=[class, fill=cyan!20]
%\tikzstyle{xzpres}=[class, fill=purple!20]
%\tikzstyle{xyzpres}=[class, fill=white]
\tikzstyle{nonpres}=[class]
\tikzstyle{xypres}=[class, bicolor rectangle,
        left color=red!20,
        right color=green!20, fill=none]
\tikzstyle{yzpres}=[class, bicolor rectangle,
        left color=green!20,
        right color=blue!20,
        fill=none]
\tikzstyle{xzpres}=[class, bicolor rectangle,
        right color=red!20,
        left color=blue!20,
        fill=none]
\tikzstyle{xyzpres}=[class, tricolor rectangle, 
         top color=green!20,
         left color=red!20,
         right color=blue!20, fill=none]
\matrix[row sep=1.3cm,column sep=.07cm] {
& & & & & \node (ALL) [nonpres]{\phantom{$R_Z$}{ALL}\phantom{$R_Z$}}; & & & & &\\
& \node (CYX_P_Rx) [xpres]{$C(Y,X) + \Pauli + R_X$}; & & & & \node (CZY_P_Ry) [ypres]{$C(Z,Y) + \Pauli + R_Y$}; & & & & \node(CXZ_P_Rz) [zpres]{$C(X,Z) + \Pauli + R_Z$};&\\t
\node (CXZ_P) [xzpres]{$C(X,Z) + \Pauli$}; &\node (T4_P_Rx) [xpres]{$\T_4 + \Pauli + R_X$}; & & & \node(CYX_P) [xypres]{$C(Y,X) + \Pauli $}; & \node(T4_P_Ry) [ypres]{$\T_4+ \Pauli + R_Y$}; & & & \node (CZY_P) [yzpres]{$C(Z,Y) + \Pauli$};& \node(T4_P_Rz) [zpres]{$\T_4 + \Pauli + R_Z$}; & & &\\
& \coordinate (Above_CXX); & & & & \coordinate (Above_CYY); & & & & &\\
& \node (CXX_P_Rx) [xpres]{$C(X,X) + \Pauli + R_X$}; & & & &\node (CYY_P_Ry) [ypres]{$C(Y,Y) + \Pauli + R_Y$}; & & & & \node(CZZ_P_Rz) [zpres]{$C(Z,Z) + \Pauli + R_Z$};&\\
 \node (CXX_P) [xpres]{$C(X,X) + \Pauli$}; & \node (CXX_Rx) [xpres]{$C(X,X) + R_X$}; & \node (CXX_X_theta_yz) [xpres]{$C(X,X) + X+ \theta_{YZ}$}; & & \node(CYY_P) [ypres]{$C(Y,Y) + \Pauli$}; &\node (CYY_Ry) [ypres]{$C(Y,Y) + R_Y$}; & \node (CYY_Y_theta_xz) [ypres]{$C(Y,Y) + Y +\theta_{XZ}$}; & &\node (CZZ_P) [zpres]{$C(Z,Z) + \Pauli$}; & \node (CZZ_Rz) [zpres]{$C(Z,Z) +  R_Z$};& \node (CZZ_Z_theta_xy) [zpres]{$C(Z,Z) + Z + \theta_{XY}$};\\
& \node (CXX_X) [xpres]{$C(X,X) + X$}; & & & &\node (CYY_Y) [ypres]{$C(Y,Y) + Y$}; & & & & \node(CZZ_Z) [zpres]{$C(Z,Z) + Z$};&\\
};
\node (T4_P_Gamma)[nonpres, yshift=0, xshift=0cm] at ($(CYX_P_Rx)!0.5!(CZY_P_Ry)$) {$\T_4 + \Pauli + \Gamma$};
\node (T4_P)[xyzpres]  at ($(Above_CXX)!0.5!(Above_CYY)$) {$\T_4 + \Pauli$};

%\coordinate[above left=1cm of CXZ_P.north] (LEFT);
%\coordinate[below right=1cm of CXZ_P_Rz.south] (RIGHT);

% EDGES
\path[draw] 
(ALL) edge (CYX_P_Rx.north)
(ALL) edge (CZY_P_Ry.north)
(ALL) edge (CXZ_P_Rz.north)
(CYX_P_Rx) edge (T4_P_Rx)
(CZY_P_Ry) edge (T4_P_Ry)
(CXZ_P_Rz) edge (T4_P_Rz)
(T4_P_Rx) edge (CXX_P_Rx)  
(T4_P_Ry) edge (CYY_P_Ry)  
(T4_P_Rz) edge (CZZ_P_Rz)
(CXX_P_Rx) edge (CXX_Rx)
(CYY_P_Ry) edge (CYY_Ry)
(CZZ_P_Rz) edge (CZZ_Rz)
(CXX_Rx) edge (CXX_X)
(CYY_Ry) edge (CYY_Y)
(CZZ_Rz) edge (CZZ_Z)
(CXX_P_Rx) edge (CXX_P.north)
(CYY_P_Ry) edge (CYY_P.north)
(CZZ_P_Rz) edge (CZZ_P.north)
(CXX_P_Rx) edge (CXX_X_theta_yz.north)
(CYY_P_Ry) edge (CYY_Y_theta_xz.north)
(CZZ_P_Rz) edge (CZZ_Z_theta_xy.north)
(CXX_P.south) edge (CXX_X)
(CYY_P.south) edge (CYY_Y)
(CZZ_P.south) edge (CZZ_Z)
(CXX_X_theta_yz.south) edge (CXX_X)
(CYY_Y_theta_xz.south) edge (CYY_Y)
(CZZ_Z_theta_xy.south) edge (CZZ_Z)
(ALL) edge (T4_P_Gamma)
(T4_P_Gamma) edge (T4_P)
(T4_P_Rx.south) edge (T4_P)
(T4_P_Ry.south) edge (T4_P)
(T4_P_Rz.south) edge (T4_P)
(CYX_P_Rx.south) edge (CXZ_P.north)
(CYX_P_Rx.south) edge (CYX_P.north)
(CZY_P_Ry.south) edge (CYX_P.north)
(CZY_P_Ry.south) edge (CZY_P.north)
(CXZ_P_Rz.south) edge (CZY_P.north)
(CXZ_P.south) edge (T4_P)
(CYX_P.south) edge (T4_P)
(CZY_P.south) edge (T4_P);

\draw (CXZ_P_Rz.south) edge (CXZ_P.north);
%\draw (LEFT) edge[->] (CXZ_P.north);
%\draw (CXZ_P_Rz.south) edge[->] (RIGHT);

\end{tikzpicture}

\end{center}
\caption{The inclusion lattice of the 27 fragments of the multi-qubit Clifford operations. Here, ``ALL'' denotes every such Clifford operation, $\Gamma$ is the ``vertex rotation'' $(I - iX - iY - iZ) / 2$, and all other generators are defined in the main text. Red, green, and blue denote $X$-, $Y$-, and $Z$-preserving, respectively. See \cite{GS22} for complete details.}
\label{fig:Cliffordlattice}
% \end{sidewaysfigure}
\end{figure}
\vfill
\end{landscape}
